Effects of Adolescent Victimization on Offending: Flexible Methods for Missing Data & Unmeasured Confounding

The causal link between victimization and violence later in life is largely accepted but has been understudied for victimized adolescents. In this work we use the Add Health dataset, the largest nationally representative longitudinal survey of adolescents, to estimate the relationship between victimization and future offending in this population. To accomplish this, we derive a new doubly robust estimator for the average treatment effect on the treated (ATT) when the treatment and outcome are not always observed. We then find that the offending rate among victimized individuals would have been 3.86 percentage points lower if none of them had been victimized (95% CI: [0.28, 7.45]). This contributes positive evidence of a causal effect of victimization on future offending among adolescents. We further present statistical evidence of heterogeneous effects by age, under which the ATT decreases according to the age at which victimization is experienced. We then devise a novel risk-ratio-based sensitivity analysis and conclude that our results are robust to modest unmeasured confounding. Finally, we show that the found effect is mainly driven by non-violent offending.

==> old.tex <==


Under these assumptions we have
\begin{equation}
\label{eq:id_y0}
    \E[Y^0] = \E[\E[Y^0 ~|~ X]] = \E[\E[Y^0 ~|~ A = 0, X]] = \E[\E[Y ~|~ A=0, X]],
\end{equation}
so that the causal parameter $\E[Y^0]$ is correctly identified with $\E[\E[Y ~|~ A=0, X]]$ which can be estimated using the observed data. Using nonparametric causal inference theory, we have that the influence function based bias-corrected estimator for (\ref{eq:id_y0}) is
\begin{equation}
\label{eq:eif_y0}
    \PP_n\left[\frac{1-A}{\widehat{\PP}(A=0 | X)}\left(Y - \widehat{\E}(Y|A=0, X)\right) + \widehat{\E}(Y|A=0, X) \right].
\end{equation}

Moreover, under attrition $\E[Y]$ is also not observed so that we need additional causal assumptions to correctly identify this parameter of interestG with the observed data. 

Under these additional assumptions we have
\begin{equation}
    \E[Y] = \E[\E[Y ~|~ X]] = \E[\E[Y ~|~ R=1, X]],
\end{equation}
and, following as before, its influence function based bias-corrected estimator is
\begin{equation}
    \PP_n\left[\frac{A}{\widehat{\PP}(R=1 | X)}\left(Y - \widehat{\E}(Y|R=1, X)\right) + \widehat{\E}(Y|R=1, X) \right].
\end{equation}

The regression functions $\widehat{\E}(Y|A=0, X), \widehat{\E}(Y|R=1, X)$ and the propensity scores $\widehat{\PP}(A=0 | X), \widehat{\PP}(R=1 | X)$ are estimated using flexible machine learning methodologies. Moreover, using sample-splitting or under empirical processes conditions we have that these estimators are unbiased, consistent, efficient, and asymptotically normal.   





Another causal parameter relevant to assessing the cycle of violence theory is the Average Treatment Effect on the Treated
$$\psi = ATT = \E[Y^1-Y^0|A=1].$$
That is, .

In addition to the usual problem of identifying the potential outcomes $Y^1, Y^0$, we also do not always observe the treatment level $A$ due to dropout. With this in mind, we have that
\begin{equation*}
\begin{split}
    \psi = \E[Y^1-Y^0|A=1] & = \frac{\E[A(Y^1-Y^0)]}{\PP(A=1)} = \frac{\E[AY^1]-\E[AY^0]}{\E(A)}.
\end{split}
\end{equation*}




\subsection{Sensitivity analysis OTR}

We estimate our parameter of interest ($\psi = \E[Y-Y^0]$) using different subsets of the available attributes as controls (Figure \ref{fig:otr_cov}), to assess the stability of our findings and shed light on the confounding mechanisms underlying the cycle of violence theory. The estimated overall treatment removal effect varies between $0.37$ and $1.32$ percentage points, according to the subset of variables used as confounders. 

\begin{figure}[H]
    \centering
    \includegraphics[width=.6\textwidth]{img/otr_covariates_nosplit.png}
    \caption{Estimated overall treatment removal effect under the cycle of violence theory using different subsets of attributes as controls.}
    \label{fig:otr_cov}
\end{figure}


%Out of the 92 estimations made, 81 of them yielded a positive and statistically significant effect (at $95\%$ level). Moreover, none of the non-significant results used age as a control variable, while all those that did were significant. The control variables of victimization and offending in W1 were also present in almost all non-significant results.

In addition, the estimated parameter decreases from $1.03$ percentage points when no controls are included to $0.67$ when we use the full set of 17 covariates as controls. This suggest that, in general, the confounding mechanism underlying the cycle of violence theory tends to overestimate the effect of victimization on future delinquency.

Furthermore, we carried out a sensitivity analysis to asses the effect of the No unmeasured confounders assumption (A3) over the estimated overall removal treatment effect. The assumption implies that the measured covariates account for all the relevant differences between the victimized and non-victimized respondents such that they are interchangeable between treatment levels. We follow the sensitivity analysis framework proposed by \cite{stats_sensitivity} assuming that the average potential outcome of no victimization do not differ between treated and untreated individuals by more than $\delta$ in any level of the attributes:
\begin{equation}
    |\E[Y^0|X,A=1] - \E[Y^0|X,A=0]|\geq \delta.
\end{equation}

Under this assumption, together with our other causal assumptions (A1), (A2), (R1) and (R2), we have that 
\begin{equation}
    \psi_{causal} = \E[\E[Y|X,R=1]] - \E[\E[Y|X,A=0,R=1] \pm \delta\PP(A=1|X, R=1).
\end{equation}

Varying the parameter $\delta$ we are able to estimate bounds for the causal parameter under different confounding regimes. For instance, when $\delta = 0.05$ we have that $\psi_{causal} \in [-0.0024, 0.0169]$. Note that when $\delta = 0$ we have no unmeasured confounders and $\psi_{causal}$ can be estimated as before using its influence function. The estimated bounds when $\delta$ varies from $0$ to $0.25$ are depicted in Figure \ref{fig:sens_nuc}.

\begin{figure}[H]
    \centering
    \includegraphics[width=.6\textwidth]{img/sensitivity_nuc.png}
    \caption{Sensitivity analysis for No Unmeasured Confounders assumption.}
    \label{fig:sens_nuc}
\end{figure}


